Forecasting Action through Contact Representations from First Person Video

Human actions involving hand manipulations are structured according to the making and breaking of hand-object contact, and human visual understanding of action is reliant on anticipation of contact as is demonstrated by pioneering work in cognitive science. Taking inspiration from this, we introduce representations and models centered on contact, which we then use in action prediction and anticipation. We annotate a subset of the EPIC Kitchens dataset to include time-to-contact between hands and objects, as well as segmentations of hands and objects. Using these annotations we train the Anticipation Module, a module producing Contact Anticipation Maps and Next Active Object Segmentations - novel low-level representations providing temporal and spatial characteristics of anticipated near future action. On top of the Anticipation Module we apply Egocentric Object Manipulation Graphs (Ego-OMG), a framework for action anticipation and prediction. Ego-OMG models longer term temporal semantic relations through the use of a graph modeling transitions between contact delineated action states. Use of the Anticipation Module within Ego-OMG produces state-of-the-art results, achieving 1st and 2nd place on the unseen and seen test sets, respectively, of the EPIC Kitchens Action Anticipation Challenge, and achieving state-of-the-art results on the tasks of action anticipation and action prediction over EPIC Kitchens. We perform ablation studies over characteristics of the Anticipation Module to evaluate their utility.

==> titles.tex <==
Understanding Manipulation Actions with Contact Representations
Contact Representations for Action Understanding
Learning over Contact Representations for 
Understanding Manipulation Activity with Contact Centered Representations
Breaking Down Manipulation Activity with Contact Representations
Decomposing Manipulation Activity with Contact Representations
Structuring Manipulation Activity with Contact Centered Representations
Structuring Manipulation Activity with Contact Anticipation

Understanding Manipulation Activity with Contact Centered Representations

Understanding Egocentric Manipulation Activity with Contact Anticipation


Decomposing Manipulation Activity through Contact

Exploring Manipulation Activities through Contact Representations

Investigating Manipulation Activities through Contact Representations


Contact Anticipation for Manipulation Activities
Contact Anticipation for Manipulation Activity Understanding


Contact Anticipation for Egocentric Manipulation Video
Future 
Future Prediction through Contact Anticipation for Manipulation Activities


Future Prediction through Contact Anticipation

Future Prediction through Contact Anticipation


Determining Future Action through Contact Representations

Forecasting Action through Contact

Contact Representations for Action Forecasting
Action Forecasting with Action Representation

Action Forecasting with Contact Representations



Forecasting Action with Contact Representations
Forecasting Action employing Contact Representations
Forecasting Action applying Contact Representations
Forecasting Action adopting Contact Representations
Forecasting Action leveraging Contact Representations

Leveraging Contact Representations for Action Anticipation from First Person Video


Forecasting Action through Contact Representations
Forecasting Action through Contact Representations in First Person Video

*Forecasting Action through Contact Representations from First Person Video

Forecasting Action through Short and Long Range Contact Representations

Contact centered action representation
Contact centered action anticipation

Contact Anticipation 
Action Modeling through Contact Anticipation



\begin{itemize}
    \item We implement cite paper and conduct experiments over the augmented dataset. We use faster-RCNN trained over EPIC kitchen 400K object detection values. [should we cite the paper?] As in [cite paper] we apply the SORT tracker on the objects that are detected. We retain objects which are tracked for the last 20 frames. As described in ref[] we discard all the objects that are not tracked for the last 20 frames. Top 1 accuracy is 1.00\% for Noun classification is calculated for all the frames in the augmented dataset. Poor association of objects results in poor object tracking. As we discard objects that are not tracked for 20 frames, the number of frames having active object trackers is substantially low. The same issue persists with localization.
\end{itemize}
\begin{itemize}
Top 1 accuracy is 1.00\% for Noun classification evaluated for all the frames in validation set. Poor association of objects results in poor object tracking. As we discard objects that are not tracked for 20 frames, the number of frames having active object trackers is substantially low which results in dropping of overall accuracy. 
\end{itemize}
\begin{itemize}
Since we are using bounding boxes for localization, ground truth bounding boxes is drawn over the annotated masks. We calculate Jaccard similarity for those frames having active object trackers. Absolute Jaccard similarity is even lower than that reported in the table 4 when we consider all the frames in the validation set. 
\end{itemize}

==> useful_writing.tex <==
\iffalse

%and computing a high-level sequence of states spanning large timespans of activity.


%{\color{red} (Do we want to talk about object classifiers in here? - probably leave for Ego-OMG... Also - A different term than ``Next Active Object Prediction Network'' - the name implies that the object (category) is being predicted, rather than the segmentation of an unlabeled object)}

%{\color{red} (paragraph for Next Active Object Prediction Network - in this paragraph motivation for why segmentation is used over alternative supervision forms.)}

%{\color{red} (Paragraph on Contact Anticipation Maps)}


%{\color{red} (define terms and their relations, introduce acronyms: Contact Anticipation Module; Contact Anticipation Network; Next Active Object Prediction Network; Contact Anticipation Map; <some term for the output of Next Active Object Prediction Network>. Use figure 1, with more naming annotations, as illustration of relation between terms.)}

\subsection{Baselines}
Below we describe the baselines - whose results are given in Table \ref{table:next_active_object_prediction_results} - against which we compare our approach.

\subsubsection{Anticipation Maps - RGB}
A vanilla FCN8 architecture processes a single RGB frame and outputs two channels. One is a binary probability mask, where contact, '1', is defined as any pixel belonging to the body of a directly contacted object. The second channel is a positive-valued output of estimated time values for each pixel. We find this division to perform better than the prediction of a single-channel value of times. We merge the two channels into one by superimposing the contacted pixels of the contact segmentation map over the positive valued time map, making for a single channel output of non-negative time values. The two channels are trained in conjunction with one another, where $L = L_{BCE} + \gamma * L_1$, where $\gamma$ = 0.2.

\subsubsection{Anticipation Maps - RGB + Flow}
The FCN8 architecture of Figure \ref{fig:arch2} is modified to take optical flow rather than contact anticipation map input, where the flow channels are fed through three convolutional layers before being summed with the RGB appearance-based branch. We exclude the prediction of hand localization, for an output matching Figure \ref{fig:arch1}.


\subsubsection{Next Active Object - Center Bias}
This baseline comes from the assumption that the next active object most commonly appears near the center of the frame. We consider a fixed Gaussian at the center of each image of size (55, 55) to be the next active object. We find this size to reach the highest intersection over union of the next active object.

\subsubsection{Next Active Object - Saliency}
This baseline comes from the state of the art on saliency prediction, where a model estimates the most salient regions of an image in an RGB image. We apply pre-trained weights on the best-performing saliency benchmark on our dataset, the DeepGaze II model \cite{Kummerer_2017_ICCV}.

%\subsubsection{Next Active Object - Anticipation Maps}
%A vanilla FCN8 architecture processes a stack of 5 contact anticipation frames and outputs a single channel binary mask of pixels belonging to the next active object.

\subsubsection{Next Active Object - RGB}
A vanilla FCN8 architecture processes a single RGB frame and outputs a single channelled binary probability mask of pixels belonging to the next active object.

\subsubsection{Next Active Object - RGB + Flow}
The FCN8 architecture is modified with an additional branch of 3 optical flow input frames in the same way as Figure \ref{fig:arch2}, with a binary probability mask of pixels belonging to the next active object.

\subsubsection{Next Active Object - Multiple RGB Frames}
The FCN8 architecture is fed N = 4 RGB frames, to predict a binary probability mask of pixels belonging to the next active object.


\subsection{Discussion}
We perform experiments over three splits of our data: General; Novel Objects; Novel Persons, and report the results in Table \ref{table:next_active_object_prediction_results}. We address the issue of generalizability described earlier in section \ref{subsec:contact_anticipation_network} with these splits. 

In the General split, we include all actions \textit{Put}, \textit{Reach} and \textit{Open}, and divide splits among subjects - 21 individuals binned into training, 3 into validation, and 3 into testing. The Novel Person split is the same, restricted to only the \textit{reach} action. The Novel Object split divides the data by object categories, with 92 categories binned into training, 21 into validation, and 29 into testing, and is restricted to the \textit{reach} action.
As seen in Table \ref{table:next_active_object_prediction_results} we have observed that our model augmented with contact anticipation map inputs performs better than all the baselines. As seen in Figure \ref{fig:output_t}, the contact anticipation network with flow performs well at forecasting the expected time of contact, with an average error of 0.34 seconds when the hand is 1 second away from the object. As expected, the farther away the person is from the object, the higher the anticipation error due to the ambiguity in future activity on the part of the actor. The RGB only model performs consistently better than RGB + Flow, which shows that the flow is as informative a cue for forecasting future activity. 



%We conclude with several ablation studies over Ego-OMG w.r.t the components of the Anticipation Module.



%A surpassing of the state-of-the art with a full action understanding framework - Ego-OMG - built upon the proposed Anticipation Module, achieving \nth{1} and \nth{2} place on the unseen and seen test sets respectively of the EPIC Kitchens Action Anticipation Challenge. 




%using proposed representations within Ego-OMG ... state-of-the-art
%-classifiying actions before their start and / or completion
%-signal (based on cogsci work?)
%-Antcipation module
%  -CAM
%  -NAO seg
%-Full understanding framework - ego-omg (emphasis: built upon Anticiaption Module)
%  -Leverage egocentric perpsective (2 observable hands)
%  -Structure long video into a graph that captures longer term relations' %(structure embedded through GCN)
%  -
%-Surpass state-of-the-art
%-Evaluate utility of characteristics of Anticipation Module through ablation studies isolating those characteristics.



%We leverage the anticipation to reduce representations of video to capture structured relations between

{\color{red} (List experiments, describe, contextualize, relate, motivate)}

{\color{red} (rename and introduce acronym for Contact Anticipation Module?)}

%questions that arise in evaluating the utility of leveraging our contact anticipation maps.

%
\begin{enumerate}
    \item Experiments intro
        \item (subsubsec) EPIC Kitchens dataset
        \item (subsubsec) Contact Anticipation Module Training Splits
        \item (subsubsec) Action anticipation/prediction
    \item Ego-OMG Action Anticipation Challenge
    \item Contact Anticipation Map Evaluation
    \item Next active object prediction evaluation
    \item Ablations of contact anticipation maps and next active object prediction
\end{enumerate}


%We find that a combination of two loss terms works best, where $L = L_{BCE} + \gamma * L_1$. The contact anticipation network outputs two channels: One channel that outputs a binary segmentation mask of pixels belonging to the body or contacted objects, and another channel that regresses positive time values for each pixel. The loss for the contact anticipation network in equation is composed of two terms: The first loss term is the binary cross entropy loss  between the ground truth and estimated contact distribution(over the first channel of the network output) , and the second loss term is the L1 Norm between the ground truth and estimated time to contact(second channel of the network output). The two losses are used in conjunction with one another.


%{\color{red} Change title}

%Here we propose novel contact-centered representations of action, inspired by pioneering works in cognitive science on the studies

%The future forecasting of contact events provides near-future


%Human actions involving hand manipulations are structured according to the making and breaking of hand-object contact - we introduce representations and models for action understanding centered on contact. 

%Human actions involving hand manipulations are structured according to the making and breaking of hand-object contact - we introduce representations and models centered on contact, which we then use in classifying actions before their start and / or completion.


%Anticipation of near future actions is a necessary ability for fluid human interaction. Particularly, we are interested in anticipating the next object of interaction --- \textit{next active object anticipation}. We introduce a novel supervisory signal inspired from classic studies in neuroscience on the encoding of intentionality in human reaching movements {\color{red} (Extend this sentence into a full paragraph on neurosci / cogsci)}. Our approach stands in contrast to many other action anticipation methods for next active object anticipation in that we are not dependent on the accurate performance of object detectors or hand trackers. We focus on egocentric video for the advantages it provides w.r.t. hand manipulation action. Our model consists of two components: 1) a component for \textit{contact anticipation maps}: a mapping of pixels to a distribution of possible contact times, 2) a mapping of RGB pixels and a history of contact anticipation maps to a localization of the next active object. The conjunction of these two yields a prediction of when contact will occur, and where it will occur. We compare our approach against multiple baselines, and demonstrate superior performance. Contact anticipation maps provide information that is of utility to applications of action understanding, particularly interaction.



Table \ref{table2} shows that flow generalizes better in contact anticipation map prediction. 

We have visualized in Figure \ref{fig:output} the output of both networks on the clips across the dataset we have collected, and have shown in Figure \ref{fig:object_split_ouputs} the output of both networks on object nouns unseen during training. The contact anticipation maps contain inconsistent background predictions.
%The arrival of large-scale egocentric video datasets offer opportunities to build intelligent systems with enhanced understandings of the semantics of action. First-person videos expose important mid-level cues such as hand formation and object proximity, cues often unobservable in the third-person paradigm due to severe occlusion. In this paper we introduce a novel supervisory signal inspired from classic studies in neuroscience on the encoding of intentionality in human reaching movements. Our idea is to anticipate contact events leveraging \textit{time to contact} as supervision to learn an implicit representation of long-term hand trajectory for atomic reach and place actions. We demonstrate the success of our system on inferring hand motion profiles and predicting contact events. Furthermore, we demonstrate the utility of modeling hand motion trajectory by training our network to perform online anticipation of the next active object, showing promising results for the application of these contact anticipation maps for other applications in action understanding.
\begin{table}

  \centering

\begin{tabular}{l*{3}c}

\toprule
Evaluation & MAE & CS \\ 
\midrule 
RGB   & 0.26/0.26/0.21   & 0.19/0.23/0.21     \\ 
RGB + Flow       & \textbf{0.17}/\textbf{0.21}/\textbf{0.19}    & \textbf{0.23}/\textbf{0.26}/\textbf{0.24} \\ 
\bottomrule
\end{tabular}
\vspace{1em}
\caption{Contact anticipation map prediction results. The Mean Average Error (MAE) is reported for ground truth pixels with t $>$ 0, the Contact Segmentation (CS) is the IOU between the ground truth contacted objects and the model's predictions, and Temporal Coherence (TC) is a measure of the average error in the model's predictions between two consecutive frames. $\updownarrows$ indicates higher/lower is better.}
\label{table2}
\end{table}
%We introduced a novel supervisory signal we call "contact anticipation maps"; a hand-centered representation of visual space that captures when contacts are expected to occur for each pixel in a given image. Together with an object anticipation network, we have demonstrated a framework that captures when and were contacts are anticipated to occur. Our experiments show our contact anticipation maps have outperformed all baselines as well as performed better in generalizing to novel objects and persons. In the future we plan to explore expanding upon this framework to recognize and anticipate higher-level sequences of activity.\\

%\subsection{Motion Profile Estimation}
%The second is an evaluation of how well the incorporation of history helps in anticipating future hand-object interactions, especially under situations in which the anticipation of the next object of interest is under-constrained without temporal context, i.e. the hand is reaching for an object behind many other close objects. We introduce two baselines to evaluate this : One baseline with no recurrence (a single-frame input UNet segmentation architecture) and another UNet baseline with optical flow frames concatenated across the channels.

%\subsection{Generalizability}
%\label{subsec:contact_anticipation_network}
%The next is a test of generalizability to unknown objects. Learning to anticipate future interactions with novel objects enable our proposed model to generalize to everyday household environments filled with endless clutter and background objects. We test this with by cross-validating on the object split using the noun annotations accompanying each clip in the dataset. The next is a test of generalizability to unknown persons, as general factors such as height, weight, age, time of day, etc., can contribute in various ways to their motion profiles in day to day tasks.



%\subsection{Contact Anticipation Maps}
%The ability to convert a visual stream into a series of discrete contact transitions indicating the making and breaking of contact between the fingertips and the object, or an object in hand and another object/surface has enormous value for downstream tasks in action understanding and robotics.

%Detecting contact is difficult due to the severe occlusion between the body of the actor and the object. Leveraging a history of observations helps, due to the \textit{no force at a distance} principle. There are strict requirements that object motion is accompanied by force, and that force can only be transmitted directly via contact. Object motion is a vital cue for detecting contacts in video, and so representations of motion such as optical flow are naturally helpful for detecting contact transitions.

%Finally, we conclude with a demonstration of our network's ability to decompose a video of arbitrary length into discrete contact transitions. We do this by using the contact anticipation outputs at locations estimated to be the next active object, using the optical flow to project the anticipation maps forward in time, capturing the transition from $t > 0 \rightarrow t = 0$, or the making of contact. We demonstrate promising results for the representation of these discrete events in figure \ref{fig:contact_transition}  and leave the representation of more complicated sequential actions to future work.


%\begin{figure*}[t]
%\centering
%\includegraphics[width=\textwidth]{figure1.png}

%\label{fig:figure1}
%\end{figure*}
%detection of either the object category or the category of the action being performed.
%Focusing on the object to be acted upon without relying on the semantics of that object or action has a key advantage: 

%{\color{red} (Paragraph motivating contact - include work from cogsci / neurosci?)}


%A low level, generalizable method for action anticipation is the focus of this paper.
%\color{blue} (May want to expand this? Give a reference from cogsci paper?)}

%Guiding otjhers in their actions benefits from understanding others’ actions before their completion, and providing guidance sooner rather than later.

%If we are collaborating with someone on a task on which we are an expert yet the other is a non-expert, we can for example provide feedback based simply on reaching actions, telling the one we collaborate with as they begin an action whether it is the correct action. Providing this early response reduces both the physical load and the cognitive load, as well as reducing the completion time of the task by cutting out the remaining portion of the incorrect actions.

%Task knowledge can be engineered into our agents to an expert level, but unless our agents are capable of dynamically understanding and preempting the actions humans perform then this knowledge cannot fluidly be applied in guiding humans.


%As robots evolve in sophistication and the range of domains in which they come into contact with humans expands, it becomes increasingly important that methods for fluid interaction between humans and robots be developed. A central ability on which humans rely for interaction, yet which robots for the most part lack, is a theory of intention of the other humans with which we interact. Because we are able to anticipate the likely actions of those we interact with we are able to preempt those actions with our own, and interact fluidly on tasks.

%– if we had to wait for others’ actions to be completed before understanding the action being performed and responding accordingly then collaboration would involve excessive wait times. Concurrency in collaboration is desirable, and understanding actions before their completion is necessary for this.
%{\color{red} Add Figure with RGB image, contact anticipation map output, next active object output as input, hand-centered representation, and output}

%{\color{red} (merge prediction and anticipation motivation)} %{\color{blue} (CHECK)}

% predicting the outcome of ongoing actions



%localizing the present within the span of a large temporal horizon of an ongoing activity serves as a powerful temporal constraint on the near future. Previous approaches to action anticipation do not attempt to model these long-term temporal semantics - we do so with Egocentric Object Manipulation Graphs (Ego-OMG), aggregating the representations from the anticipation model and iteratively computing a high-level transcript over large timespans of roughly 45 seconds of activity.

%{\color{red} (context, then task description, then description of Ego-OMG)}

%{\color{red} (Motivate need for structured representation of video? Mix with motivation for contact?)}

%{\color{red} (In motivation, make novelty of Ego-OMG clear)}
%{\color{blue} (do we really want to draw a distinction here? These seem are naturally grouped into the same task: classify an action before its completed.)}

%{\color{red} Paragraph about evaluation, which ablations studies we're using, why we're using them, and what they demonstrate (ablation  over  training signal;  and  ablation  of  characteristics  in  representation  produced from that signal)}

%{\color{red} Paragraph about results, and Epic Kitchens Challenge}

%The nodes of this graph structure are then represented as vectors taken from a word embedding {\color{red} (ref)}, and embedded into a vector space through use of the GCN. The output of this graph component is then fed into an LSTM, allowing Ego-OMG to span longer time frames than the Action Module, and thus capture longer temporal dependencies and context. The final output of the LSTM constitutes the output of the GCN stream.
%there is a bell-curved shape to the velocity profile of guided hand movements.

%As such, we stress the utility of capturing this hand-centric cue ignored at large by the computer vision community.

%Inspired by these findings, we propose contact anticipation maps - a hand centered representation of visual space.

%Contact Anticipation Maps are a fine-grained estimation of pair-wise non-negative distance values between the hand and each observed point belonging to the scene.


%The Anticipation Module produces representations useful for action understanding.
%To evaluate the utility of the Anticipation Module's representations, we feed them into Ego-OMG, and evaluate their conjunction . {\color{red} We leverage these representations aggregated over large temporal horizons to localize ongoing actions within activities with Egocentric Object Manipulation Graphs (Ego-OMG).}

%{\color{red} Context - Talk about how contact events are extracted using anticipation module, how we're able to use that to model longer segments of video, and how we evaluate anticipation module w.r.t Ego-OMG performance }
%{\color{red} (Two paragraphs on how Ego-OMG is constructed (first paragraph talking about how output of both predictions (contact anticipation maps and next active object predictions) are used to create states for each video, from which a consolidated graph is created). Second paragraph talking about combined architecture (graph embedded through GCN, short-term video captured through CSNs) for action prediction/anticipation)}
%{\color{red} Replace paragraph: Contact Anticipation Maps are the product of the first network, and the input of the object network - they are not the training signal for either network}
%Xie et al \cite{xie2017learning} infer the hidden goals and intentions of the actors involved before predicting the actions they planned to take. More recent approaches apply this to to first-person perspective, modelling human behavior with MPDs and inverse reinforcement learning. Rather than explicitly model the intention of the actor, (Find intention modelling that is explicit)
writing that may be useful for later: 
correlation between long-term velocity profiles and intentionality in reaching movements  
We demonstrate our modelling of egocentric hand movements enables the learning of hand-object proximity, and utilize it 
next-active-object segmentation is likely easier because objects are always near the center of the field of view in egocentric vision. But time map estimation is likely much harder because of the geometric and semantic cues it has to reason about
understanding the interaction from both the human perspective and the object perspective is important for the
anticipation as well as to object segmentation
can help us model both the human perspective and object perspective in the view of the actor rather than the observer in the third person view.
The formation of contact of the hand with the object usually indicates that the object has become active compared to the rest of the objects in the scene. 
Similarly, the instant of contact of a tool like a knife, hammer in the hand becomes a natural transition between actions. 
Usually, any action like pick up, open or drink begins with the time of contact with the object. Similarly, any action like take, grasp, poke or press ends at the time of contact with the object. The instant of contact of hand and object naturally acts
 These moments can be used as a temporal attention mechanism
 Segmenting, recognizing or anticipating the active object in the scene can further provide attention to other action recognition, action anticipation tasks.
 the object to be segmented is a large and clear distinction between foreground and background can be obtained. 
 Experiment 2 : Test generalization to novel people for each of the baselines.
Experiment 3 : Test generalization to novel objects.
Experiment 4 : Predict contact events using predicted time masks by taking IOU of model output of image where t=0 and predicted objects from pretrained object detector. Likely only qualitative.
We apply the Fully Convolutional FCN8 architecture, a fully end-to-end hierarchical recurrent segmentation architecture that first encodes each frame using a Resnet-101 model pretrained on ImageNet. The features are fed at different resolutions to Conv-LSTM blocks, followed by bilinear upsampling operations to output a segmentation mask for each frame. We modify the output of the architecture by adding an additional branch of convolutions, making for a two-stream output of segmentation and contact anticipation maps respectively.
. The first is the Mean Average Error between the predicted anticipation time and the ground truth anticipation time, and the second is a temporal coherency loss, implemented as the Mean Average Error between the elapsed time of two consecutive frames and the difference of the network's output across two consecutive frames. The video in this case is 30 fps, making the elapsed time between two frames 0.03 seconds. 
Recent approaches of video object segmentation have been influenced by the availability of Berkeley 
Jain et al noticed a strong relation between objects and actions, using an object classifier to infer the action involved from a single static frame. ...
Copy Pasta: Spelke & Van de Valle (93) describe a series of experiments showing that infants aged 7.5 to 9.5 months are sensitive to a wide range of visual events derived from causal constraints on motion. They posit that three basic principles are active in motion understanding by late infancy: contact, cohesion, and continuity.The principle of contact equates physical
connectedness with causal connectedness: “no actionat a distance, and no contact without action.”• The principal of cohesion equates object integritywith individuality: “no splitting, no fusing.” Thisguarantees that the identity of objects remains stableover time, unless a series of causal events combinestwo objects into one (e.g., via attachment) or splits
one into two (e.g., via extraction).• The principle of continuity guarantees object solidity:“no gapped trajectories, no contactless collisions.”Objects must occupy every point along theirtrajectory (including a connected path behind anything
that occludes their motion), and no two objecttrajectories can occupy the same space at the sametime without inducing a contact relation.Interestingly, infants show fluent application of theseconstraints well before they can reliably segment still
objects, leading to the speculation that aspects ofappearance that remain invariant between causal eventscould be used to scaffold the acquisition of gestalts used togroup surfaces and boundaries.
Video object segmentation approaches can be broadly categorized into two main categories.1) one which works on static images 2) takes temporal information into consideration.
[8] adopts a CNN trained for semantic segmentation on images to a video object segmentation. [8] introduces one-shot video object segmentation by using just the ground truth segmentation mask of the first frame in the video. [9] extended [8] by using online adaptation to deal with new objects that can come in the video which are not present in the first frame. [10] proposed to synthesize more training data by generating future frames from the segmented mask in the first image. Optical flow and image have been combined effectively to learn the moving as well as static objects in videos in [10]. [11] uses a modulator to segment out objects in videos from a segmentation network. [19] jointly learn segmentation and optical flow by iteratively optimizing over it. [20] show that optical flow can be combined appearance to jointly segment objects in videos.
Video Segmentation Dataset (2011) [1], SegTrack (2013) [2], FreiburgBerkeley Motion Segmentation Dataset (2014) [3], DAVIS (2016- 2017) [5, 6], YouTubeVOS (2018) [7]. Most of the video object segmentation approaches developed for single or multiple object segmentation are for third-person videos. Egocentric datasets like Charades Egocentric dataset[], GTEA dataset and EPIC kitchen dataset[] have been designed for action recognition, action anticipation challenges. We use part of the EPIC kitchen dataset in our experiments. 
In order to segment or even recognize the object that was manipulated in an egocentric video,  modeling the interaction of hand and object is paramount. Previously there are some approaches that attempted to get an attention map of the object interaction[12,13,14,15,16]. [12] proposes to implicitly learn the region of object interactions by learning to anticipate affordance actions. [13] predicts interaction hotspots by jointly modeling motoric attention and visual attention in egocentric videos. However, there are very few attempts to produce segmentation masks of objects that were interacted by hand in egocentric hand. We attempt to utilize the hand trajectory and distance between hand and object that has been manipulated to anticipate and segment the active object of interaction. 
Poleg et al perform a temporal segmentation using egocentric motion into composable tokens of motion classes in outdoor scenarios, such as walk, run, stop, drive, etc. We believe this approach to enable the same partition of video into discrete contact events indicating the making and breaking of contact.
Many algorithms[] for detecting or segmenting objects involving human-object interaction are designed to work on images. Temporal information in videos can help to a large extent in localizing such objects of interaction. However, the problem of video object segmentation when it comes to human-object interaction is rarely studied. Video object segmentation[] in the past has mostly been evaluated for the third person viewpoint on the Berkeley Video Segmentation Dataset (2011) [1], SegTrack (2013) [2], FreiburgBerkeley Motion Segmentation Dataset (2014) [3], DAVIS (2016- 2017) [5, 6], YouTubeVOS (2018) [7]. In many of these videos there is a clear distinction between the foreground and background segmentation. Moreover, there is very little camera motion in some of these datasets and optical flow on its own plays an important clue in segmenting objects.  In this paper, we focus on the interaction of objects with the hand rather than the entire human body restricting the field of study. We further consider egocentric data to model it. However, egocentric data poses different challenges like camera motion or occlusion where the hand or the object that is manipulated isn’t visible in the entire video. We present an approach that specifically deals with it by modeling these conditions.
Generally, a video object segmentation network utilizes a segmentation mask as supervision. There are three paradigms in video object segmentation. In the first scenario, a segmentation mask is provided in all the frames in the video. In the second scenario, a segmentation mask is provided in the first frame of the video.  The last scenario is most challenging when no segmentation masks are provided.  In this paper, we are considering the last scenario often referred to as zero-shot video object segmentation Specifically, when it comes to zero-shot manipulated object segmentation in videos we need to learn to anticipate the future behavior of humans. 
Using an egocentric view to use for object anticipation is someway helpful as we are capturing the field of view of the actor. Action anticipation or object anticipation is sometimes modeled by the probability of that action occurring based on previous actions and the context. However, such a way of modeling out anticipation is not generalizable beyond the trained setting. If we have to purely consider an unsupervised way of anticipating the active object we have to consider the hand trajectory to estimate the most likely active object in the scene. 
In the study of human-object interaction, capturing the hidden goals and intentions of the actor as well as the affordances of the objects involved in these interactions are of significant importance to applications in computer vision and robotics. 
The synchronous coordination of eye, head and hand movements is well-studied among several classic studies in neuroscience. The egocentric paradigm enables the incorporation of these cues along with others such as full-body cues and object proximity, all highlighting the regions of significant importance where interactions are most likely to occur.
We further demonstrate the ability of our network to infer contact transitions and the respective labels of the objects in contact. Determining class labels corresponding to the contacted object can be difficult due to the aforementioned occlusion. However, we reap from the benefits of having access to object anticipation, utilizing a simple detection scheme where we compute an exponential weighting of the confidence score of the next active object, with the weighting determined by the time elapsed relative to the time of contact.
Hands are the driving force of change in the physical world; the onset motion and shape formation of the hands can be a useful cue into understanding the intentions of the actor. 
Yang et al classified hands based on their functional grasp type, stacking a classifier on top of the learned representations to infer the intentionality behind the actions. 
Affordances are essential to understand as they reveal the functionality of objects and the actions that can be performed with them. The problem of affordance detection is a problem well-studied in computer vision and robotic perception. An important question lies in the problem of affordance representation. Earlier representations of object affordances attempted to combine physical and material attributes with visual attributes extracted from an image, suffering from a lack of scalability due to brittle knowledgebases. Later works attempted to utilize multi-modal sensory cues such as force or depth. Many other works involve parsing visual frames into alternative representations such as skeletal pose, object trajectories, and applied forces, from which the involved affordance classes of the objects in situ can be inferred.
While many recent approaches to affordance learning phrase it as a semantic segmentation problem, fewer consider grounding the learning of affordances into direct observation of human interaction. Nagarajan et al and Fang et al learn affordance regions by learning mappings between input videos of objects in action and static templates of the corresponding objects when inactive. Xiao et al propose a Dual Attention Network model, utilizing objects to determine where particular actions are most likely to occur and vice-versa. Our approach falls into this category, where the manipulation activity of the actor is used to localize the most likely regions of future interaction.
 . The localization of contacts on Consider a pair of scissors; without any anticipation as to the semantics of the anticipated grasp, multiple future actions such as place, move, cut, or hand-off are possible. The localizing of the contacts along the handle or the blade requires the ability to have learned semantically rich cues, enabling the enhanced discrimination between the possible action classes afforded to a particular object. 
 
%a map, with a 1-1 correspondance to the pixels in the image, containing: 1) segments for hands, which take the value 0, 2) segments for next active object, which take the value time remaining to contact, and 3) segments for background, which take the value -1.

%a mapping from hand and object segmentations to time to contact.

%Training over this signal yields an architecture which, given an egocentric image with hands, shows the time to contact of the remaining positions in the image. 


% Anticipation of human action is a key component of interaction - whether human / human or human / robot interaction.


%The egocentric perspective to these hand-object interactions provides us a clear view of the situation of the actor, allowing us to exploit the proximity principle[], where "things that matter are close, and things that are close matter". Given that the body is constantly observable, kinematic priors inform us of where the hand is in relation to the environment. By situating perception from the perspective of the actor, additional advantages are gained by focusing only on what the actor is looking at rather than the entire scene when looked at from the third-person viewpoint. 

%The spatial position of the hand serves as a form of attention in locating the region of interaction of the action. Contact transitions can be an important cue for capturing key events over time, as the engagement and disengagement of objects serve as a powerful temporal attention mechanism that indicate the beginning and end of their accompanying actions. Object-centric actions such as take, open, drink, grasp, poke, cut, etc each have moments of importance indicated by the formation and breakage of contact between the hand and the respective object. Contact transitions naturally serve as a way to segment long, unconstrained video into discrete and distinct fine-grained moments of importance. In this paper we propose a method for detecting and anticipating both \textit{where} the contacts are expected to happen, and anticipating \textit{when} they happen.
We include clips in which the motor plan of a directed movement is abruptly cancelled in favor of another, i.e. somebody reaches for a tomato, realizes he/she has nothing to put it on, and instead grabs the neighboring tray. This inclusion enables the learning of contextual cues more advanced than hand-object proximity. We do not include annotations of objects unintentionally contacted, i.e. somebody bumps into a spoon while reaching a knife. 
By training our model on the estimated time of contact, our model may use the hand-object proximity.
We utilize a similar definition of the next active object to that of [][], with the requirement that the next active object is to be either directly contacted by the person or indirectly contacted by an object held by the person.
We also aim to answer the question of how well our model is able to anticipate interactions with objects of different affordances; our ground truth anticipation maps reveal that objects are accompanied by motion profiles of varying durations based on the required accuracy of the hand's motion, a finding extensively replicated throughout many experiments in neuroscience. 
 We also provide an analysis of our model's performance on action segments of unusual duration, testing the ability of our network to infer the changing goals and intentions of the person.
%Most existing approaches to the anticipation of object interaction either rely on tracking hands, objects, or both. Other approaches require additional forms of supervision, such as prior knowledge of the objects pre-interaction. Considering this, we propose a novel form of supervision which we refer to as contact anticipation maps. Contact anticipation maps are a fine-grained representation of the time-to-contact between the hand and each object/surface in the scene. Figure 1 shows sample anticipation maps of several types of directed reaching movements between the hand and the object. 
, with three relevant scenarios shown in Figure 1. In Figure 1a), a person reaches for the handle of the door, with the anticipation maps reflecting the estimated time to arrival towards the object. Figure 1b) shows the person placing a pot on the surface of the table, with the anticipation maps reflecting the anticipated time remaining to complete the put action. Figure 1c) shows a person bringing a knife to a carrot, with the anticipation maps reflecting the estimated time for the two objects to make contact.


%By training our model on the estimated time of contact, our model essentially learns a hand-centric distance function based not only on hand-object proximity but object semantics as well. By leveraging a history of these contact anticipation maps, our model is able to use the estimated trajectory of the aimed movement in forecasting future hand-object interactions. To demonstrate the utility of these contact anticipation maps, we apply them in the task of next active object prediction, where we train two networks; a contact anticipation network, that separately processes a history of video frames to output a stack of contact anticipation maps, each of which are recurrently fed to the object anticipation network, which predicts the next target of a guided hand movement. We demonstrate the utilization of this novel supervisory signal significantly improves performance on the anticipation of the next active object in unconstrained egocentric video.
\fi






%As hand position is tracked through time in Contact Anticipation Maps, we train the Contact Anticipation Network to localize hand trajectory within the broader bell-shaped motion profile captured through learning over the dataset of point-to-point hand movements exhibiting this phenomenon.







%The utility of the anticipation module for downstream tasks in action understanding lies in its separation of objects in the scene into three distinct categories - active objects (objects currently contacted by the actor), next-active objects (objects most likely to be contacted in the near future), and non-active objects - objects not predicted to come into contact with hands in the near future.

%By restricting ourselves to the representation of objects either currently or expected to come in contact with the hands, we rule out 'background' objects that play no role in the actions performed, effectively using the hands as an attention mechanism. This is of great benefit to environments of high clutter and complexity (such as EPIC Kitchens), where previous methods relying on an exhaustive list of candidate object proposals are likely to fail {\color{red]} (reference?)}.


%. 4) By restricting ourselves to the representation of objects either currently or expected to come in contact with the hands, we rule out 'background' objects that play no role in the actions performed.

%3) As the motion profile of hand movements captured in 3D space provides a means of inferring the endpoint of point-to-point hand movements through the underlying bell-shaped phenomena, likewise a history stack of contact anticipation maps provides a means of implicitly estimating the pixels belonging to the target entity of point-to-point hand movements.






%Contact Anticipation Maps provide several benefits: 1) The predicted Contact Anticipation Maps can be thresholded at arbitrarily small time values (e.g. $t = 0.01$) to arrive at a binary segmentation mask of the hands along with the objects currently engaged in activity with them. 2) Similarly, by thresholding the contact anticipation maps at mid-range time values (e.g. $0.01 < t < 0.5$, we arrive at near-future candidates of possible interaction. 3) As the motion profile of hand movements captured in 3D space provides a means of inferring the endpoint of point-to-point hand movements through the underlying bell-shaped phenomena, likewise a history stack of contact anticipation maps provides a means of implicitly estimating the pixels belonging to the target entity of point-to-point hand movements. 4) Finally, the mask associated with the hands, objects of interaction, and near-future objects of possible interaction can be incorporated as a form of attention for end-to-end video architectures in action anticipation. We demonstrate all three aforementioned use-cases of the contact anticipation maps throughout the experiments conducted in this paper.


%Over these mappings we train a network, the product of which is a contact anticipation map: a distribution over each pixel in the image of potential time to contact. 

%Finally, the contact anticipation maps can directly be fed as inputs to an end-to-end video architecture for tasks pertaining to action understanding. 
%^As localizing the hand along the time axis of a bell-shaped motion profile serves as an extremely useful discriminator between candidate near-future objects of interaction, our contact anticipation maps can likewise be aggregated over time t

%{\color{red} (Remove/compress this) This stands in contrast to the majority of existing methods for anticipating the next active object. These methods function through an understanding of the semantic relations involved in the activity being performed as well as explicit modeling of the hand trajectory – these methods fail when objects or hands cannot be accurately recognized and tracked, and it fails in tasks and for object categories over which it has not be trained}.


%In modelling the distance between hands and objects belonging to the environment, we propose contact anticipation maps, a hand-centered representation of visual space. Contact anticipation maps encode a distribution of time-to-contact values for each pixel belonging to the scene. We utilize contact anticipation maps as a hand-centric distance function, stacking contact anticipation maps over time to implicitly represent the trajectory of the hand.


%-Neuroscience reaching experiments
%-Distribution of times (across CAM; across distributinos of reaching)
%-Leverages hands (is hand centric)
%-Includes hands
%    - We discriminate the activity of the left hand from the right hand by modelling each hand separately; as such, our contact anticipation network produces two separate channels, one channel for each hand.
%    - output separate channels for left and right hand
%-Foreground, background?
%    -Of importance to the contact anticipation network are relations not only of hand-object distance, but the semantics and affordances of the objects involved. 
%    -Contact anticipation Network captures not only the distance between the hand and entities, but also the semantics of the entities involved - objects of different  semantic notions of distance - Time to contact relies not only on hand distance to a particular entity, but the nature 
%-Reference to cogsci paper
%    -Figure from cogsci paper? Velocity distribution

%Where the Contact Anticipation Maps provide timing information relevant to near future action understanding, they do not provide explicit localization information. Both timing and localization information are relevant to action understanding. 




%Localization when combined with Contact Anticipation Maps gives both a time range for anticipated contact (sampled from a region in the Contact Anticipation Map), and the region of the object to be interacted with.

% For this we employ the Next Active Object Network, superimposing the spatial predictions of the 


%Rather than directly predict the classes of the next active object of interaction, we divide the learning between two components: A component being the next active object network, which predicts a fine-grained segmentation of pixels belonging to the next active object, and an object classifier component, being a generic object classifier trained over the EPIC Kitchens object annotations. We take this approach to leverage both training signals 


%The insight which allows us to approach the task of next active object anticipation in a low-level fashion, differing from the existing methods with their reliance on classifiers and trackers, is a novel representation {\color{red} (contact anticipation maps are not a training signal - rephrase)}: \textit{contact anticipation maps} - see figure \ref{fig:figure1}.




% We use this augmented EPIC Kitchens dataset in training the Anticipation Module.

%We circumvent the lack of availability of depth as a modality, as it typically is not adopted in mainstream egocentric Activities of Daily Living (ADL) datasets, 

%Aggregating these maps over time allows us to implicitly represent the underlying bell-shaped motion profile of the point-to-point hand movement relative to each object in the scene. See Figure {\color{red} X} for an example contact anticipation map predictions.


%We center our representations around ..., given clearly in ego-centric video. We term ... the active object, and the ... the next active object.
%In next active object ... space, time.
%... around the spatio-temporal relations in manipulation actions
%-Action centered around (next) active object
%-Ego centric perspective centered on object
%-Our representations centered on object as well
%    -time
%    -space

%As the physical interactions between hands and objects are more pronounced under the egocentric perspective, the spatiotemporal structure of manipulation actions can be exploited for action understanding. As establishment of contact with objects is the precondition for all subsequent actions that can be performed, we focus on an aspect of action anticipation - the prediction of the next active object. Simultaneously, we also capture the time at which contact with that object object will occur.

%We focus on two aspects of action anticipation: anticipation of the segmentation of  the next contacted object which the action will entail - the \textit{next active object} - and the time at which contact with that object will occur. {\color{red} (motivate why this is of utility to action anticipation / prediction)}

%The commence of a human manipulation action as seen in egocentric video is at the point of contact between the hand and the object being manipulated.

%Capturing the spatial relations between the hand and object at all times preceding the time of contact enables us to predict the next active object

%As such, to forecast future contact events allows us to capture not only the object of the next most likely action, .

%both
%-timing
%-spacial
%-active object : the object(s) currently in contact with each hand
%-next active object : The object(s) most likely to come into contact with each hand
